Performance-Robustness Tradeoffs in Adversarially Robust Linear-Quadratic Control

While $\mathcal{H}_\infty$ methods can introduce robustness against worst-case perturbations, their nominal performance under conventional stochastic disturbances is often drastically reduced. Though this fundamental tradeoff between nominal performance and robustness is known to exist, it is not well-characterized in quantitative terms. Toward addressing this issue, we borrow from the increasingly ubiquitous notion of adversarial training from machine learning to construct a class of controllers which are optimized for disturbances consisting of mixed stochastic and worst-case components. We find that this problem admits a stationary optimal controller that has a simple analytic form closely related to suboptimal $\mathcal{H}_\infty$ solutions. We then provide a quantitative performance-robustness tradeoff analysis, in which system-theoretic properties such as controllability and stability explicitly manifest in an interpretable manner. This provides practitioners with general guidance for determining how much robustness to incorporate based on a priori system knowledge. We empirically validate our results by comparing the performance of our controller against standard baselines, and plotting tradeoff curves.

==> cdc.tex <==
% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}  % Comment this line out
%                                                           % if you need a4paper
% %\documentclass[a4paper, 10pt, conference]{ieeeconf}      % Use this line for a4
%                                                           % paper

% \IEEEoverridecommandlockouts                              % This command is only
%                                                           % needed if you want to
%                                                           % use the \thanks command
% \overrideIEEEmargins
% % See the \addtolength command later in the file to balance the column lengths
% % on the last page of the document

% \usepackage{Shorthands}
% \title{Performance-Robustness Tradeoffs in Adversarially Robust Linear-Quadratic Control}

% \author{Bruce D.\ Lee*\thanks{*Equal contribution} , Thomas T.C.K.\ Zhang* , Hamed Hassani, and Nikolai Matni}

% \date{Department of Electrical and Systems Engineering, University of Pennsylvania}

% \newcommand{\citep}[1]{\cite{#1}}

% \newcounter{cdc}
% \setcounter{cdc}{1}

% \begin{document}
% \maketitle
% \input{abstract}
% \input{introduction}
% \input{adversariallyrobustcontrol}
% \input{tradeoffs}
% \input{empirical}
% \input{conclusion}

% \bibliographystyle{IEEEtran}

% \bibliography{refs}

% \end{document}

==> control.tex <==
\section{Adversarially Robust Controllers}
\label{s: adversarial robust controllers}

% In this section, we address Problem~\ref{prob:controller}.
%{\color{red} I know this section is currently illegible - just have been working through to make sure proofs are correct and such.}

In this section, we address the problem of finding an optimal controller to minimize the adversarial cost \eqref{eq:adversarialLQRobjective}. Formally, we solve Problem \ref{prob:controller}. The constraint on the adversarial budget in \eqref{eq:hardadversarialLQRobjective} makes this problem non-trivial. To summarize our approach, we first consider the problem where we replace the hard constraint on the adversarial budget with a soft constraint (a.k.a.\ regularization) via duality. However, due to the randomness in the disturbances, we cannot yet say that the hard and soft constrained formulations are equivalent. We will then argue via ergodicity that the two formulations are equivalent, and thus an optimizer to \eqref{eq:hardadversarialLQRobjective} may be found by bisection on the soft constraint parameter. 

As a first step, we will design a controller which minimizes a version of the above problem where the hard constraint on $\delta$ is removed, and a penalty on the power of the adversary is added. 
\begin{align}
    \label{eq:adversarialLQRobjective}
     \limsup_{T \to \infty} 
    \frac{1}{T} \Ex \brac{\max_{\delta \mbox{ causal}} x_T^\top Q x_T + \sum_{t=0}^{T-1} x_t Q x_t + u_t^\top R u_t - \gamma^2 \delta_t^\top \delta_t}
\end{align}
The following Lemma provides necessary and sufficient conditions for the existence of a stabilizing controller which minimizes the above objective. Similar statements in continuous time may be extracted from a more general result found in \cite{doyle1989optimal}. 

\begin{lemma}
    \label{lem:adversarial LQR sol} A controller attaining a finite objective value for  \eqref{eq:adversarialLQRobjective} exists if and only if there exists a solution to the following discrete algebraic Riccati equation   
         \begin{align}
         \label{eq:modified DARE}
        P = Q + A^\top P A - A^\top P \bmat{B & I} \paren{\bmat{B & I}^\top P \bmat{B & I} +\bmat{R \\ & -\gamma^2 I}}^{-1} \bmat{B & I}^\top P A.
        \end{align}
    such that 
    \begin{itemize}
        \item $0 \preceq P \prec\gamma^2 I$.
        %\item $I + P - PB(-\gamma^2 I + B^\top P B)^{-1}B^\top P \succ 0$. {\color{red} I believe that this condition is incorrect as stated, and the correct one is redundant.}
        \item $A + BK$ has eigenvalues in the open unit disc, where $K$ is given by
        \begin{equation}
        \label{eq:suboptimal adversarial controller}
        \begin{aligned}
            K &= -(R+B^\top M B)^{-1} B^\top M A, \\
            M &= P + P(\gamma^2 I - P)^{-1} P.
        \end{aligned}
        \end{equation}
    \end{itemize}
    As long as the above conditions are true, 
    \begin{enumerate}
        \item The controller $u_t = K x_t$ with $K$ given by \eqref{eq:suboptimal adversarial controller} minimizes the objective in \eqref{eq:adversarialLQRobjective}. \label{num:1}
        \item The optimal adversarial perturbation under the controller $u_t=Kx_t$ is given by 
        \[
            \delta_t = (\gamma^2 I - P)^{-1} P ((A+BK) x_t + w_t).
        \] \label{num:2}
        \item The objective value of \eqref{eq:adversarialLQRobjective} achieved under controller \ref{num:1} and adversary \ref{num:2} is is  $\trace(M \Sigma_w)$.
    \end{enumerate}
    %Necessity might require a nonstrict upper bound on the spectral norm of P?} 
    %{\color{red} If these conditions are not satisfied, then there does not exist a controller for which the objective value is finite. Necessity proof follows in part from Lemma 3.6 of \cite{basar1991hinf}.}
\end{lemma}

%Move Proof to Appendix, even for arxiv version

%We are now ready to find a controller which minimizes \eqref{eq:hardadversarialLQRobjective}. 
The solution approach for the above problem follows that in \cite{basar1991hinf} for minimax games. We first consider the finite horizon version of the problem, and then take the limit to reach the steady state solution presented above. The finite horizon version of the problem is solved by defining a saddle point cost-to-go function in place of the standard cost-to-go function in nominal linear-quadratic control. We then recurse backwards in time, solving an unconstrained concave quadratic maximization problem to determine the adversarial perturbation at each step, and then solving an unconstrained convex minimization problem at each step to determine the control input. It should be noted that unlike most adversarially robust machine learning problems, adversarially robust LQR provides a closed form expression for the adversarial perturbation. 

We now return our attention to the objective \eqref{eq:hardadversarialLQRobjective}. By dualizing the constraint on the adversary, and demonstrating via ergodicity that we can interchange the order of expectation with the optimization over the dual variable, we show that the original problem of interest may be solved by repeatedly solving the subproblem \eqref{eq:adversarialLQRobjective}. This is made precise in the following theorem.

\begin{theorem}
    \label{thm:adversarial controller solution}
    The problem of finding the optimal adersarially robust controller to adversary level $\varepsilon$ as in \eqref{eq:hardadversarialLQRobjective}, is equivalent to
    \begin{align*}
         \min_\gamma  \limsup_{T \to \infty} \min_{u_0, \dots, u_{T-1}}
    \frac{1}{T} \paren{\Ex \brac{\max_{\delta \mbox{ causal}} x_T^\top Q x_T + \sum_{t=0}^{T-1} x_t Q x_t + u_t^\top R u_t - \gamma^2 \delta_t^\top  \delta_t} + \gamma^2 \epsilon T}.
    \end{align*}
\end{theorem}

The above theorem provides a means to solve \eqref{eq:hardadversarialLQRobjective} via bisection in conjunction with Lemma~\ref{lem:adversarial LQR sol}.

In order to examine tradeoffs, it will also be helpful to determine clean way to express the soft and hard constrained costs of an arbitrary controller $K$ in closed form. The following corollaries provides a way to compute this. Their proofs follow the exact same approach as Lemma~\ref{lem:adversarial LQR sol} and Theorem~\ref{thm:adversarial controller solution}.

\begin{corollary}
    \label{cor:adversarial controller performance}
    For an an arbitrary stabilizing controller $u_t = Kx_t$, \eqref{eq:adversarialLQRobjective} is finite if and only if there exists a solution to the Riccati equation
    \begin{align}
        P = Q + (A+BK)^\top P (A+BK) - (A+BK)^\top P \paren{P - \gamma^2 I} P (A+BK)
    \end{align} 
    such that $ 0 \preceq P \prec \gamma^2 I$. Then 
    \begin{enumerate}
        \item The optimal adversarial perturbation for \eqref{eq:adversarialLQRobjective} under the controller $u_t = K x_t$ is given by 
        \begin{align}
            \label{eq:adversary for given controller}
            \delta_t = (\gamma^2 I - P)^{-1} P ((A+BK)x_t + w_t)
        \end{align}
        \label{num:arbitrary adversary}
        \item The objective value of \eqref{eq:adversarialLQRobjective} under controller $u_t = K x_t$ and the adversary \ref{num:arbitrary adversary} in is given by $\trace(M \Sigma_w)$, where $M = P + P(\gamma^2 I - P)^{-1} P$. 
    \end{enumerate}
\end{corollary}

% \textit{Proof:}
% The proof follows a dynamic programming argument identical to that of Lemma~\ref{lem:adversarial LQR sol}, except rather than minimizing over $u_t$ at each step, we substitute $u_t = Kx_t$. \hfill $\blacksquare$

\begin{corollary}
     The performance of a stabilizing controller $K$  at adversarial level $\epsilon$ in \eqref{eq:hardadversarialLQRobjective} may be evaluated by solving 
    \begin{align*}
         \min_\gamma  \limsup_{T \to \infty} 
    \frac{1}{T} \paren{\Ex \brac{\max_{\delta \mbox{ causal}} x_T^\top Q x_T + \sum_{t=0}^{T-1} x_t Q x_t + u_t^\top R u_t - \gamma^2 \delta_t^\top  \delta_t} + \gamma^2 \epsilon T}
    \end{align*}
    where $u_t = Kx_t$ for all $t \geq 0$. 
\end{corollary}

%\hh{let's talk about the organization of the paper whenever that we meet.}

==> introducion_old.tex <==
\section{Introduction}

Designing robust controllers has been an important focus in both the applications and theory of controls. In general, one wishes to have a controller that achieves a target goal, such as stabilization or tracking, while not succumbing to small errors or perturbations, be it through stochastic noise or systematic inaccuracies. Historically, the great majority of advances seen in control theory has been through the former objective, for example traditional PID control or Kalman's optimal control \textbf{CITE}. On the other hand, the success of doing control \textit{robustly} is a more subtle story. It has been known for a few decades now that for linear systems, when disturbances are assumed to be purely independent and identically-distributed (i.i.d.) zero-mean Gaussian noise, so-called $\calH_2$ control is optimal \textbf{CITE}. Similarly, when disturbances are assumed to be purely worst-case causal perturbations (measured in the $\calH_\infty$ signal norm), then $\calH_\infty$ control is optimal \textbf{CITE}). Despite the theoretical power of $\calH_\infty$ control, it has generally been observed that $\calH_\infty$ control performs poorly in practice due to its over-conservatism \textbf{CITE}. On the other hand, $\calH_2$ controllers have generally seen success in practice, but suffer greatly from deviations away from zero-mean Gaussian disturbances, as well as a fundamental lack of robustness guarantees on the resulting closed-loop system, e.g.\ the seminal and succinct example in \cite{doyle1979robustness}.

There have certainly been efforts to bridge the practical effectiveness of $\calH_2$ and the theoretical robustness guarantees of $\calH_\infty$. Perhaps the most well-known approach is the mixed $\calH_2$-$\calH_\infty$ method, which solves a $\calH_2$ subproblem subject to a robust stability constraint. It is generally understood (\textbf{CITE?}) that there exists a trade-off between performance and robustness, where nominal performance is measured by the controller's cost on the system with zero-mean i.i.d.\ Gaussian disturbances. However, a key feature missing from the analyses of methods that interpolate between the stochastic and worst-case settings is guarantees on how much nominal performance is traded off for robustness in interpretable, meaningful system-theoretic quantities. Such guarantees are integral to the general applicability of robust control. Given the understanding that robust control methods will generally perform worse in non-pathological settings, the most important insight robust control can provide to practitioners, perhaps more so than the controller synthesis itself, is characterizing \textit{when} robustness is necessary based on \textit{a priori system knowledge}.

Toward establishing rigorous bounds on a performance-robustness tradeoff, we look toward the burgeoning area of adversarial robustness in machine learning, where the goal is to design classifiers that are robust to small perturbations to the data. Recently, there has been work looking into rigorously analyzing the various performance-robustness tradeoffs in adversarially robust learning, including precise characterizations of the generalization errors of standard versus adversarially trained models under the random features model \citep{javanmard2020precise, hassani2022curse}, and ``no free lunch'' theorems for the existence of robust models \citep{tsipras2018robustness, dohmatob2019generalized}. Robust machine learning and robust control share many of the same overarching goals--however, one key feature that distinguishes the results of the two is that adversarial robustness does not throw away stochasticity in the min-max framework, and thus performance-robustness tradeoffs in the nominal stochastic setting versus the worst-case settings can be traced out by varying the power of the adversary relative to the stochastic noise. We formulate a smooth interpolation between the stochastic $\calH_2$ and worst-case $\calH_\infty$ settings by analyzing \textit{adversarially robust control}.

\subsection*{Our Contributions}

We consider an adversarial setting for infinite-horizon linear-quadratic control, where the adversary enters as a norm-bounded perturbation to the state aiming to maximize the LQR cost. We note that this adversarial perturbation is introduced on top of additive stochastic noise, and can in fact depend on the noise realizations causally. As stated, this becomes a non-trivial problem, as the form of the adversary becomes dependent on the noise realizations, and thus the relative power of a fixed norm-bound becomes seemingly stochastic. This is what distinguishes our framework from $\calH_\infty$ and similar settings, where stochastic disturbances are encompassed into the search for the worst-case disturbance to the unperturbed system. This search will inevitably reach an impasse, where the power given to worst-case disturbance must in theory be large in order to subsume the stochastic noise, leading to over-conservative control policies. The benefit of approaching the problem through the adversarial lens is that it allows us to separate the worst-case component from the stochastic. 

To address the possible non-stationarity of the solution to the adversarial problem, we demonstrate through strong duality and ergodicity that the adversarial min-max problem can be turned into a regularization parameter, where the regularization parameter is \textit{independent of the noise realization}. We then derive through dynamic programming arguments the precise form of the adversarial disturbance as well as the corresponding optimal controller, both directly resulting from the solution of a particular Algebraic Ricatti Equation. This in fact establishes a direct correspondence between adversarially robust control and the so-called $\gamma$-suboptimal $\calH_\infty$ (\textbf{CITE}) problem.

Now armed with the precise form of adversary, we derive bounds on the performance-robustness tradeoff of the resulting adversarially-robust controller. Our main tools are adaptations of perturbation bounds from system identification literature \cite{mania2019certainty}, which allow us to find quantitative upper and lower bounds on the LQR cost gap between the adversarially-robust and nominal controller. In particular, we show that system-theoretic terms manifest naturally, which provides straight-forward interpretations for how system properties affect the performance-robustness tradeoff.

Lastly, we provide numerous experiments demonstrating the effectiveness of the adversarially robust controller across various settings, ranging from pure stochastic to pure worst-case noise. We show that in many cases, adversarially robust controllers perform close to the better of two worlds between $\calH_2$ and $\calH_\infty$.


\subsection*{Related Work}

Adversarial stuff in RL, robust control lit duh, distributional (?) robustness in control


% mention that there is no free lunch theorems for adversarial robustness that don't exist for control


% Adv robust control is hard question b/c the eps-worst case disturbances depend causally on the realization of the stochastic noise, thus the gain of a disturbance sequence is a random variable.
\paragraph{Notation:} 

==> problem_formulation.tex <==
\section{Problem Formulation}
{\color{red} Combine sections 2 and 3? Would look like 
\begin{itemize}
    \item Introduce nominal and adversarial costs
    \item Provide known optimizer for nominal cost
    \item Provide optimizer for adversarial cost
    \item Leave any discussion of Tradeoffs for the following section
\end{itemize}
}
Consider a fully observed linear-time-invariant (LTI) system with state  disturbances composed of both stochastic and adversarial components: let $x_t \in \R^n$ be the system state, $u_t \in \R^m$ the input, $w_t \in \R^n$ and $\delta_t \in \R^n$ the stochastic and adversarial components of the process disturbance, respectively. The initial condition and stochastic component of the process noise are assumed to be i.i.d.\ zero-mean Gaussians: $x_0 \sim{} \calN(0,\Sigma_0)$, $w_t \overset{\mathrm{i.i.d.}}{\sim} \calN(0,\Sigma_w)$. The LTI system is then defined by the following equation:
\begin{equation}\label{eq:ss}
    \begin{aligned}
     x_{t+1} &= Ax_t + Bu_t + w_t + \delta_t.
\end{aligned}
\end{equation}
It is assumed that $\mathbf{\delta}$ may not depend on state information or the components of the stochastic noise that will come in the future. This notion is made precise in the following definition.

%\hh{define precisely what "causal" means.} 
\begin{definition}(Causality)
    We say that the sequence $\delta$ is \emph{causal} if for all $t \geq 0$, $\delta_t$ is a function only of states $x_0, \dots, x_t$ and stochastic disturbances $w_0, \dots, w_t$. 
\end{definition}

We let $Q \succeq 0$ be a weight matrix for the state cost, and $R \succ 0$ be a weight matrix for the input cost. We will consider the infinite horizon objective 
\[
    \limsup_{T\to\infty} \frac{1}{T} \Ex \brac{x_T^\top Q x_T + \sum_{t=0}^{T-1} x_t^\top Q x_t + u_t^\top R u_t}
\]
subject to the dynamics \eqref{eq:ss}. If the adversary is assumed to be zero, i.e. $\delta_t = 0$ for all $t \geq 0$, then minimizing the above objective reduces to the nominal LQR problem. If we instead assume that the adversary has power bounded by $\varepsilon$, then we end up with an adversarially robust LQR problem. We will denote these two objectives by $\NC$ for the nominal cost and $\AC$ for the adversarial cost, as follows:
\begin{align}
     \label{eq:nominal_cost}
    \NC(\bfu) &= \limsup_{T \to \infty} 
    \frac{1}{T} \Ex \brac{ x_T^\top Q x_T + \sum_{t=0}^{T-1} x_t Q x_t + u_t^\top R u_t}, \quad x_{t+1} = Ax_t + Bu_t + w_t \\
    \label{eq:hardadversarialLQRobjective}
    \AC(\bfu)  &= \limsup_{T \to \infty} \frac{1}{T} \Ex \brac{\max_{\substack{\mathbf{\delta} \mbox{ causal} \\ \norm{\mathbf{\delta}}_{\ell_2}^2 \leq T \varepsilon}} x_T^\top Q x_T + \sum_{t=0}^{T-1} x_t^\top Q x_t + u_t^\top R u_t}, \quad x_{t+1} = Ax_t + Bu_t + w_t + \delta_t
\end{align}

% We will design a controller to minimize the adversarial cost (AC)
% \begin{align}
    
%     \AC(\curly{u_t}_{t\geq0}) =  \limsup_{T \to \infty} 
%     \frac{1}{T} \Ex \brac{\max_{\substack{\delta \mbox{ causal} \\ \norm{\delta}_{\ell_2}^2 \leq T \epsilon}} x_T^\top Q x_T + \sum_{t=0}^{T-1} x_t^\top Q x_t + u_t^\top R u_t}
% \end{align}

% This is in contrast to the nominal linear quadratic regulation problem, which considers the nominal cost (NC)
% \begin{align}
   
%     \NC(\curly{u_t}_{t\geq0}) =  \limsup_{T \to \infty} 
%     \frac{1}{T} \Ex \brac{ x_T^\top Q x_T + \sum_{t=0}^{T-1} x_t Q x_t + u_t^\top R u_t}
% \end{align}
%where the state progresses according to \eqref{eq:ss} with $\delta_t = 0$ for $t = 0, 1, 2, ...$. 

In order to ensure that the there exists a stabilizing controller, and that minimizing the objective \eqref{eq:nominal_cost} {\color{red} or \eqref{eq:hardadversarialLQRobjective}!} provides a stabilizing controller, we make the following assumption.
\begin{assumption}\label{assumption: stabilizable detectable}
    $(A, B)$ is stabilizable, $(Q^{1/2},A)$ is detectable. 
\end{assumption}
This assumption is standard for LQR. Requiring that $(A,B)$ is stabilizable ensures that a stabilizing controller exists, while assuming that $(Q^{1/2}, A)$ is detectable ensures that if any component of the state becomes large, it is reflected in the cost. 
Under this assumption, there exists a nominally stabilizing state feedback control law $u_t = K x_t$ minimizing \eqref{eq:nominal_cost}, where
\begin{align}
    \label{eq:lqr}
    K = -(R + B^\top P B)^{-1} B^\top P A 
\end{align}
and $P$ is the solution to the Discrete Algebraic Riccati Equation (DARE) 
\[
    P = Q + A^\top P A - A^\top P B(R + B^\top P B)^{-1} B^\top P A.
\]

It is shown in \cite{doyle1978guaranteed} that a soft constrained version \eqref{eq:hardadversarialLQRobjective} is minimized by a central $\calH_\infty$ solution. Our first objective is to supply a solution to the hard-constrained version of this problem in \eqref{eq:hardadversarialLQRobjective}. We also provide a new proof for the solution of the soft-constrained problem by viewing it through the lens of mixed stochastic/deterministic dynamic games \cite{basar1991hinf}.
{\color{red} Rather than stating this as a problem here, we should just provide a solution here. Title section ``Adversarially Robust control''. }

\begin{problem} \normalfont{(Adversarially Robust Control)}. 
    \label{prob:controller}
    Determine a controller $\bfu$ which minimizes the objective \eqref{eq:hardadversarialLQRobjective}.
\end{problem}

Secondly, we will we will investigate the interplay between the two objectives \eqref{eq:nominal_cost} and \eqref{eq:hardadversarialLQRobjective}. In particular, if we allow an adversary a budget of $\varepsilon$, then we expect that a controller chosen to minimize \eqref{eq:hardadversarialLQRobjective} will achieve a higher cost when evaluated on \eqref{eq:nominal_cost} relative to the controller minimizing \eqref{eq:hardadversarialLQRobjective}. As an example of this, consider the simple 2-d integrator system.
\begin{align*}
    x_{t+1} = \bmat{1 & 1 \\ 0 & 1} x_t + \bmat{0 \\ 1} u_t + w_t + \delta_t
\end{align*}
where $w_t \sim \calN(0, I)$. We consider an adversarial level $\varepsilon = 0.1$. If we vary $\varepsilon$ from $0$ to $0.1$, and minimize the objective \eqref{eq:hardadversarialLQRobjective}, we achieve a collection of different controllers which are robust to different levels of adversary. Evaluating the performance of these controllers under the adversarial level $\varepsilon = 0.1$ and $\varepsilon = 0$ results in the following tradeoff curve.


%In particular, if a controller is designed to optimize objective \eqref{eq:hardadversarialLQRobjective}, how much extra cost is incurred for the objective \eqref{eq:nominal_cost} beyond that of the nominal LQR controller \eqref{eq:lqr}. 


\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/intro_tradeoff_curve.pdf}
    \caption{Example of tradeoffs for 2-d integrator system. }
    \label{fig:my_label}
\end{figure}


For an adversarial level $\varepsilon$, it is useful to understand how severe the above tradeoff curve is. In particular, we will study the gap between the nominal costs of an adversarially robust LQR controller and a nominal LQR controller. 
\begin{problem}\normalfont{(Tradeoff analysis)}
    \label{prob:tradeoff}
    Determine upper and lower bounds on the gap between the nominal cost of the adversarially robust controller resulting from Problem~\ref{prob:controller} and the LQR controller \eqref{eq:lqr} as a function of system theoretic quantities. 
\end{problem}

Our results show that the bounds on the nominal cost gap have a critical dependence upon the controllability of the system. Here, we will briefly review controllability. 
\begin{definition}
    An $n$ dimensional LTI system defined by the tuple $(A,B)$ is said to be \textnormal{controllable} if for any $x_0, x \in \R^n$, there exists some sequence of inputs $u_0, \dots, u_{n-1}$ such that when applied to the system in the absence of noise starting from state $x_0$, we reach state $x$.  
\end{definition}
\begin{definition}
    An \textnormal{$\ell$- step controllabilty matrix} is
    \begin{align*}
    \calC_\ell = \bmat{B & AB & \dots & A^{n-1} B}
\end{align*}
\end{definition}
\begin{definition}
    The \textnormal{controllability gramian} is defined as
    \[
        W_c(A,B) = \lim_{\ell \to \infty} \calC_\ell \calC_\ell^\top = \sum_{t=0}^\infty A^t B B^\top (A^t)^\top 
    \]
\end{definition}
\begin{lemma}
The following conditions are equivalent
\begin{itemize}
    \item $(A,B)$ controllable
    \item $\rank(\calC_n) = n$
    \item $W_c(A,B) \succ 0$
\end{itemize}
\end{lemma}

{\color{red} Discussion about the svs of the controlalbility grammian, and their implication}

%To answer this question, we first supply a solution to \eqref{eq:hardadversarialLQRobjective}, which is of independent interest.





%\hh{I typically avoid "want to" and use "Our goal is" or "we aim to" or "we will characterize/study/investigate" etc }



% \begin{problem} \normalfont{(Adversarially Robust Control)}. 
%     \label{prob:controller}
%     Determine a causal controller ($u_t$ depends only on $\curly{x_k}_{k \leq t}$) which minimizes the objective \eqref{eq:hardadversarialLQRobjective}.
% \end{problem}

% The solution to this problem is presented in Theorem~\ref{thm:adversarial controller solution}. {\color{red} Just move this theorem up here... it will make the subsequent components of the problem formulation easier to write.} It turns out to be a central suboptimal $\calH_\infty$ controller at a level determined by $\varepsilon$. Interestingly, this level also depends upon the covariance of the noise, $\Sigma_w$. 



% Write $\NC(K)$ to represent $\NC(\curly{u_t}_{t \geq 0})$ where $u_t = K x_t$ for all $t \geq 0$, and similarly for $\AC(K)$. 
% \begin{problem} \normalfont{(Bounding the nominal cost gap)}. 
    % Let $K_\epsilon$ be the state feedback controller which minimizes \eqref{eq:hardadversarialLQRobjective} and let  $K$ minimize \eqref{eq:lqr}. Determine upper and lower bounds on $\NC(K_\epsilon) - \NC(K)$.
% \end{problem}

% The gap will be characterized in terms of several system theoretic properties, recapped below. 

% {\color{red} Introduce relevant quantities.}

